Sharper Bounds on Four Lattice Constants

The Korkine--Zolotareff (KZ) reduction, and its generalisations, are widely used lattice reduction strategies in communications and cryptography. The KZ constant and Schnorr's constant were defined by Schnorr in 1987. The KZ constant can be used to quantify some useful properties of KZ reduced matrices. Schnorr's constant can be used to characterize the output quality of his block $2k$-reduction and is used to define his semi block $2k$-reduction, which was also developed in 1987. Hermite's constant, which is a fundamental constant lattices, has many applications, such as bounding the length of the shortest nonzero lattice vector and the orthogonality defect of lattices. Rankin's constant was introduced by Rankin in 1953 as a generalization of Hermite's constant. It plays an important role in characterizing the output quality of block-Rankin reduction, proposed by Gama et al. in 2006. In this paper, we first develop a linear upper bound on Hermite's constant and then use it to develop an upper bound on the KZ constant. These upper bounds are sharper than those obtained recently by the authors, and the ratio of the new linear upper bound to the nonlinear upper bound, developed by Blichfeldt in 1929, on Hermite's constant is asymptotically 1.0047. Furthermore, we develop lower and upper bounds on Schnorr's constant. The improvement to the lower bound over the sharpest existing one developed by Gama et al. is around 1.7 times asymptotically, and the improvement to the upper bound over the sharpest existing one which was also developed by Gama et al. is around 4 times asymptotically. Finally, we develop lower and upper bounds on Rankin's constant. The improvements of the bounds over the sharpest existing ones, also developed by Gama et al., are exponential in the parameter defining the constant.

==> micros.tex <==
\usepackage{amsmath}
\usepackage{amsfonts}
\usepackage{amssymb}
\usepackage{algorithm}
\usepackage{algorithmic}
\usepackage{graphicx}
\usepackage{verbatim}
\usepackage{amsthm}
\usepackage{xcolor}
\usepackage{multirow}

%\usepackage{mathtools} \mathtoolsset{showonlyrefs}

\newtheorem{Remark}{Remark}
\newtheorem{Algorithm}{Algorithm}[section]
\newtheorem{THEOREM}{THEOREM}[section]
% \newtheorem{theorem}{Theorem}
\newtheorem{lemma}{Lemma}
% \newtheorem{remark}{Remark}
\newtheorem{claim}{Claim}
\newtheorem{corollary}{Corollary}
% \newtheorem{example}{Example}
% \newtheorem{definition}{Definition}

% Equations:
\newcommand{\beq}{\begin{equation}}
\newcommand{\eeq}{\end{equation}}
\newcommand{\beqnn}{\begin{equation*}}
\newcommand{\eeqnn}{\end{equation*}}
\newcommand{\beqy}{\begin{eqnarray}}
\newcommand{\eeqy}{\end{eqnarray}}
\newcommand{\beqynn}{\begin{eqnarray*}}
\newcommand{\eeqynn}{\end{eqnarray*}}
\newcommand{\bit}{\begin{itemize}}
\newcommand{\eit}{\end{itemize}}
\newcommand{\ben}{\begin{enumerate}}
\newcommand{\een}{\end{enumerate}}
\newcommand{\bex}{\begin{example}}
\newcommand{\eex}{\end{example}}

% Algorithm

\newcommand{\balg}[1]{\begin{algorithm} \caption{#1}}
\newcommand{\ealg}{\end{algorithm}}

\newcommand{\balgc}{\begin{algorithmic}[1]}
\newcommand{\ealgc}{\end{algorithmic}}

% Arrays, Matrices and Tables:
\newcommand{\bary}{\begin{array}}
\newcommand{\eary}{\end{array}}
\newcommand{\bmx}{\begin{bmatrix}}
\newcommand{\emx}{\end{bmatrix}}
\newcommand{\bsmx}{\left[\begin{smallmatrix}}
\newcommand{\esmx}{\end{smallmatrix}\right]}
\newcommand{\bmxc}[1]{\left[\begin{array}{@{}#1@{}}}
\newcommand{\emxc}{\end{array}\right]}
%position
\newcommand{\bcn}{\begin{center}}
\newcommand{\ecn}{\end{center}}

% To give an extra space above say \bar{b} under an hline:
\newcommand{\clear}[1]{\mathrel{\raisebox{-.50ex}{$#1$}}}
% use (on the matrix row following the \hline):  \clear{\bar{b}}
% or just use: \mathrel{\raisebox{-.75ex}{$\bar{b}$}}

\newcommand{\red}[1]{\textcolor{red}{#1}} % Red text alert style

% Matrix related:
\newcommand{\diag}{\mathrm{diag}}
\newcommand{\rank}{\mathrm{rank}}

%Dimension of matrices:

\newcommand{\cve}[1]{{#1 \times 1}}
\newcommand{\rve}[1]{{1 \times #1}}
\newcommand{\Rbb}{{\mathbb{R}}}
\newcommand{\Zbb}{{\mathbb{Z}}}
\newcommand{\Cbb}{{\mathbb{C}}}

%\newcommand{\kbk}{{k \times k}}
\newcommand{\nbk}{{n \times k}}
\newcommand{\nbn}{{n \times n}}
\newcommand{\nbm}{{n \times m}}
\newcommand{\nbp}{{n \times p}}
\newcommand{\mbm}{{m \times m}}
\newcommand{\mbn}{{m \times n}}
\newcommand{\mbp}{{m \times p}}
\newcommand{\pbn}{{p \times n}}
\newcommand{\pbp}{{p \times p}}
\newcommand{\mbmmn}{{m \times (m-n)}}
\newcommand{\bigO}{{\mathcal{O}}}

\newcommand{\Rk}{\Rbb^{k}}
\newcommand{\Rm}{\Rbb^{m}}
\newcommand{\Rn}{\Rbb^{n}}
\newcommand{\Rp}{\Rbb^{p}}
\newcommand{\Rkbk}{\Rbb^{k \times k}}
\newcommand{\Rnbk}{\Rbb^{n \times k}}
\newcommand{\Rnbn}{\Rbb^{n \times n}}
\newcommand{\Rnbm}{\Rbb^{n \times m}}
\newcommand{\Rnbp}{\Rbb^{n \times p}}
\newcommand{\Rmbm}{\Rbb^{m \times m}}
\newcommand{\Rmbn}{\Rbb^{m \times n}}
\newcommand{\Rmbp}{\Rbb^{m \times p}}
\newcommand{\Rpbn}{\Rbb^{p \times n}}
\newcommand{\Rpbm}{\Rbb^{p \times m}}
\newcommand{\Rpbp}{\Rbb^{p \times p}}
\newcommand{\Rmbmmn}{\Rbb^{m \times (m-n)}}
\newcommand{\Cn}{\Cbb^{n}}
\newcommand{\Cmbn}{\Cbb^{m\times n}}
\newcommand{\Zm}{\Zbb^{m}}
\newcommand{\Zn}{\Zbb^{n}}
\newcommand{\Zmbn}{\Zbb^{m \times n}}
\newcommand{\Znbn}{\Zbb^{n \times n}}


% Statistical Material:
\newcommand{\pro}[1]{\mathcal{P}\{ #1 \} }
\newcommand{\Exp}[1]{\mathcal{E}\{ #1 \} }
\newcommand{\cov}[1]{\mathrm{cov}\{#1\}}
\newcommand{\cnd}{\kappa}

% Special symbols:

\newcommand{\sA}{{\scriptscriptstyle A}}
\newcommand{\sE}{{\scriptscriptstyle E}}
\newcommand{\sss}{\scriptscriptstyle }
\newcommand{\sLS}{{\scriptscriptstyle \text{LS}}}
\newcommand{\sILS}{{\scriptscriptstyle \text{ILS}}}
\newcommand{\sRLS}{{\scriptscriptstyle \text{RLS}}}
\newcommand{\sOL}{{\scriptscriptstyle \text{OL}}}
\newcommand{\sOB}{{\scriptscriptstyle \text{OB}}}
\newcommand{\sOR}{{\scriptscriptstyle \text{OR}}}
\newcommand{\sB}{{\scriptscriptstyle \text{BL}}}
\newcommand{\sD}{{\scriptscriptstyle \text{D}}}
\newcommand{\sL}{{\scriptscriptstyle L}}
\newcommand{\sS}{{\scriptscriptstyle S}}
\newcommand{\sV}{{\scriptscriptstyle V}}
\newcommand{\sR}{{\scriptscriptstyle \text{R}}}
\newcommand{\sBB}{{\scriptscriptstyle \text{BB}}}
\newcommand{\sBR}{{\scriptscriptstyle \text{BR}}}
\newcommand{\sBL}{{\scriptscriptstyle \text{BL}}}
\newcommand{\sBBL}{{\scriptscriptstyle \text{BBL}}}
\newcommand{\sBBS}{{\scriptscriptstyle \text{BBS}}}
\newcommand{\sBBV}{{\scriptscriptstyle \text{BBV}}}
\newcommand{\sBBBD}{{\scriptscriptstyle \text{BBBD}}}
\newcommand{\sOBL}{{\scriptscriptstyle \text{OBL}}}
\newcommand{\sOBS}{{\scriptscriptstyle \text{OBS}}}
\newcommand{\sOBV}{{\scriptscriptstyle \text{OBV}}}
\newcommand{\sOBBD}{{\scriptscriptstyle \text{OBBD}}}


\newcommand{\mbbR}{{\mathbb{R}}}
\newcommand{\mbbZ}{{\mathbb{Z}}}

%Bold
\newcommand{\A}{\boldsymbol{A}}
\newcommand{\B}{\boldsymbol{B}}
\newcommand{\C}{\boldsymbol{C}}
\newcommand{\D}{\boldsymbol{D}}
\newcommand{\E}{\boldsymbol{E}}
\newcommand{\F}{\boldsymbol{F}}
\newcommand{\G}{\boldsymbol{G}}
\renewcommand{\H}{\boldsymbol{H}}
\newcommand{\I}{\boldsymbol{I}}
\newcommand{\J}{\boldsymbol{J}}
\newcommand{\K}{\boldsymbol{K}}
\renewcommand{\L}{\boldsymbol{L}}
\newcommand{\M}{\boldsymbol{M}}
\newcommand{\N}{\boldsymbol{N}}
\renewcommand{\P}{\boldsymbol{P}}
\newcommand{\Q}{\boldsymbol{Q}}
\newcommand{\R}{\boldsymbol{R}}
\renewcommand{\S}{\boldsymbol{S}}
\newcommand{\T}{\boldsymbol{T}}
\newcommand{\U}{\boldsymbol{U}}
\newcommand{\V}{\boldsymbol{V}}
\newcommand{\W}{\boldsymbol{W}}
\newcommand{\X}{{\boldsymbol{X}}}
\newcommand{\Y}{{\boldsymbol{Y}}}
\newcommand{\Z}{\boldsymbol{Z}}
\renewcommand{\a}{\boldsymbol{a}}
\renewcommand{\b}{\boldsymbol{b}}
\renewcommand{\c}{\boldsymbol{c}}
\renewcommand{\d}{\boldsymbol{d}}
\newcommand{\e}{\boldsymbol{e}}
\newcommand{\f}{\boldsymbol{f}}
\newcommand{\g}{\boldsymbol{g}}
\newcommand{\h}{\boldsymbol{h}}
\renewcommand{\l}{\boldsymbol{l}}
\newcommand{\n}{\boldsymbol{n}}
\newcommand{\p}{\boldsymbol{p}}
\newcommand{\q}{\boldsymbol{q}}
% We have to define bold r in the following way, otherwise there would be a problem
\newcommand{\rr}{\boldsymbol{r}}
\newcommand{\s}{\boldsymbol{s}}
\renewcommand{\u}{\boldsymbol{u}}
\renewcommand{\v}{\boldsymbol{v}}
\newcommand{\w}{\boldsymbol{w}}
\newcommand{\x}{{\boldsymbol{x}}}
\newcommand{\y}{{\boldsymbol{y}}}
\newcommand{\z}{\boldsymbol{z}}
\newcommand{\0}{{\boldsymbol{0}}}

%bar
\newcommand{\bd}{{\bar{d}}}
\newcommand{\bl}{{\bar{l}}}
\newcommand{\bx}{{\bar{x}}}
\newcommand{\by}{{\bar{y}}}
\newcommand{\bz}{{\bar{z}}}
\newcommand{\bc}{{\bar{c}}}
\newcommand{\br}{{\bar{r}}}
%barbold

\newcommand{\bbz}{{\bar{\z}}}
\newcommand{\bby}{{\bar{\y}}}
\newcommand{\bbx}{{\bar{\x}}}
\newcommand{\bbL}{{\bar{\L}}}
\newcommand{\bbD}{{\bar{\D}}}
\newcommand{\bbQ}{{\bar{\Q}}}
\newcommand{\bbR}{{\bar{\R}}}
\newcommand{\bbu}{{\bar{\u}}}
\newcommand{\bbl}{{\bar{\l}}}

%tilde
\newcommand{\tA}{{\tilde{A}}}
\newcommand{\tE}{{\tilde{E}}}
\newcommand{\td}{{\tilde{d}}}
\newcommand{\tr}{{\tilde{r}}}
\newcommand{\tv}{{\tilde{v}}}
\newcommand{\ty}{{\tilde{y}}}

%tildebold
\newcommand{\tbD}{{\tilde{\D}}}
\newcommand{\tbL}{{\tilde{\L}}}
\newcommand{\tbP}{{\tilde{\P}}}
\newcommand{\tbQ}{{\tilde{\Q}}}
\newcommand{\tbl}{{\tilde{\l}}}
\newcommand{\tbR}{{\tilde{\R}}}
\newcommand{\tby}{{\tilde{\y}}}

%check
\newcommand{\cba}{{\check{\a}}}
\newcommand{\cbx}{{\check{\x}}}
\newcommand{\cbz}{{\check{\z}}}

%hat
\newcommand{\ha}{{\hat{a}}}
\newcommand{\hr}{{\hat{r}}}
\newcommand{\hx}{{\hat{x}}}
\newcommand{\hz}{{\hat{z}}}
%hatbold
\newcommand{\hbG}{{\hat{\G}}}
\newcommand{\hbR}{{\hat{\R}}}
\newcommand{\hba}{{\hat{\a}}}
\newcommand{\hbc}{{\hat{\c}}}
\newcommand{\hbd}{{\hat{\d}}}
\newcommand{\hbr}{{\hat{\r}}}
\newcommand{\hbw}{{\hat{\w}}}
\newcommand{\hbx}{{\hat{\x}}}
\newcommand{\hby}{{\hat{\y}}}
\newcommand{\hbz}{{\hat{\z}}}


% Special format:
\newcommand{\bSigma}{{\boldsymbol{\Sigma}}}
\newcommand{\bxi}{\boldsymbol{\xi}}
\newcommand{\bmu}{\boldsymbol{\mu}}
\newcommand{\brho}{\boldsymbol{\rho}}
\newcommand{\sign}{\mathrm{sign}}
\newcommand{\fnl}{{\mathcal{F}}}
\newcommand{\huber}{{\mathcal{H}}}
\newcommand{\6}{{\partial}}
\newcommand{\8}{{\infty}}
\newcommand{\4}{{\nabla}}

%functions
\providecommand{\norm}[1]{\lVert#1\rVert}
\providecommand{\round}[1]{\lfloor#1\rceil}
\providecommand{\rnd}[1]{\lfloor #1 \rceil}
%\providecommand{\abs}[1]{\left| #1 \right|}

\renewcommand{\top}{{\mkern-1.5mu\mathsf{T}}}
\newcommand{\hem}{{\mkern-.8mu\mathsf{H}}}

